Speculative Beam Search for Simultaneous Translation

Beam search is universally used in full-sentence translation but its application to simultaneous translation remains non-trivial, where output words are committed on the fly. In particular, the recently proposed wait-k policy (Ma et al., 2019a) is a simple and effective method that (after an initial wait) commits one output word on receiving each input word, making beam search seemingly impossible. To address this challenge, we propose a speculative beam search algorithm that hallucinates several steps into the future in order to reach a more accurate decision, implicitly benefiting from a target language model. This makes beam search applicable for the first time to the generation of a single word in each step. Experiments over diverse language pairs show large improvements over previous work.

==> Makefile <==
.PHONY: dvi ps pdf all space clean veryclean distclean

#SHELL = /bin/sh
#MAKE  = gmake

# latex --interaction {batchmode, nonstopmode, scrollmode, errorstopmode}
#TEX = latex --interaction batchmode
TEX = latex 

######################################################################
# source files

texfiles = $(wildcard *.tex)
bibfiles = $(wildcard *.bib *.bst)

tblfiles = $(wildcard tbl/*.tex)

styfiles  = $(wildcard *.sty *.cls)

figfiles  = $(wildcard figures/*.fig)
figfiles += $(wildcard figures/*.plt)
figfiles += $(wildcard diagram-*.pdf)
figfiles += $(wildcard figures/*.tex)
figfiles += $(wildcard figures/*.ps)
figfiles += $(wildcard figures/*.epsi)
figfiles += $(wildcard figures/*.c)
figfiles += $(wildcard figs/*.eps)
figfiles += $(wildcard figs/*.gnuplot)
figfiles += $(wildcard figs/*.mp)
figfiles += $(wildcard figs/*.pdf)
figfiles += $(wildcard figs/*.tex)


figfiles += $(wildcard figures/apps/*.fig)
figfiles += $(wildcard figures/apps/*.plt)
figfiles += $(wildcard figures/apps/*.pdf)
figfiles += $(wildcard figures/apps/*.ps)
figfiles += $(wildcard figures/apps/*.epsi)
figfiles += $(wildcard figures/apps/*.c)

tmp_files = $(wildcard *.log)
tmp_files += $(wildcard *.aux)
tmp_files += $(wildcard *.blg)
tmp_files += $(wildcard *.bbl)
tmp_files += $(wildcard *.toc)
tmp_files += $(wildcard *.dvi)
#tmp_files += (texput.log)

######################################################################
# output files

target =main

######################################################################
# make targets

all:  pdf

simple:
	latex ${target}; dvips -t letter ${target}.dvi -o ${target}.ps


dvi: ${target}.dvi

ps: ${target}.ps

pdf: ${target}.pdf

space:
	@if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	@-/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps

clean veryclean distclean:
	if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps ${target}.dvi

######################################################################
# rules

%.dvi : %.tex
	@if [ -d fig ]; then cd fig; ${MAKE} all; fi
	@${TEX} $<
	@if  grep citation ${*F}.aux ; then \
		bibtex ${*F};	\
		${TEX} $<;	\
		bibtex ${*F};	\
	fi
	@${TEX} $<
#	@-/bin/rm -f ${tmp_files}

%.ps : %.dvi
	dvips -t letter -P pdf -G0 -q -o $@ $<

#%.pdf : %.ps
#	ps2pdf $< $@
#	~/local/macscripts/refresh.scpt

#	cd figs; mptopdf *.mp; cd ..

# %.pdf: %.tex ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles}
# 	pdflatex ${*F} #> ${*F}.log
# 	#tail ${*F}.log
# 	@if  grep Citation ${*F}.log ; then \
# 		bibtex ${*F};   \
# 		pdflatex ${*F};      \
# 		bibtex ${*F};   \
# 		pdflatex ${*F}
# 	#fi
# 	#open $@
# #	~/local/macscripts/refresh.scpt


%.pdf : %.tex ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles}
	@if [ -d fig ]; then cd fig; ${MAKE} all; fi
	#pdflatex si
	pdflatex $<
	@if  grep citation ${*F}.aux ; then \
		bibtex ${*F};	\
		pdflatex $<;	\
		pdflatex $<;	\
	fi
	@-/bin/rm -f ${tmp_files}
	#pdfcrop --margin "5 5 5 5" main.pdf
	# open main-crop.pdf

long.bib:	all.bib
	./remove-short.pl all.bib > long.bib


######################################################################
# dependences

${target}.dvi: ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles} Makefile

paper.pdf:	${target}.pdf
	gs -q -sPAPERSIZE=letter -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -dFirstPage=1 -dLastPage=12 main.pdf

si.pdf:	${target}.pdf
	gs -q -sPAPERSIZE=letter -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -dFirstPage=13 -dLastPage=20 main.pdf




==> exp_new.tex <==
% !TEX root = main.tex

\section{Experiments}

\begin{table}[!]\centering
\begin{tabular}{|l|c|c|c|c|c|c|}\hline
Beam  & 1     & 2     & 3     & 4      & 5 \\\hline
 3 &   35.82  & 36.35 & 35.79 & 36.58  & 36.27 \\\hline
 5 &   36.12  & 36.43 & 35.89 & 36.11  & 35.88 \\\hline
 7 &   36.11  & 36.60 & 35.60 & 36.15  & 35.99 \\\hline
 10 &  36.00  & 36.77 & 35.94 & 36.10  & 36.23 \\\hline
 15 &  36.00  & 36.58 & 35.68 & 36.42  & 35.96 \\\hline
\end{tabular}
\caption{Zh-En 4-ref dev BLEU w/ wait-1 model}
\label{tab:w1}
\end{table}


\begin{table}[!]\centering
\begin{tabular}{|l|c|c|c|c|c|c|}\hline
Beam  & 1     & 2     & 3     & 4      & 5 \\\hline
 3 &   31.92  & 32.64 & 32.69 & 33.44  & 34.19 \\\hline
 5 &   31.00  & 32.31 & 33.42 & 33.62  & 33.54 \\\hline
 7 &   31.08  & 32.13 & 32.52 & 32.81  & 33.71 \\\hline
 10 &  31.07  & 32.05 & 32.82 & 32.72  & 33.33 \\\hline
 15 &  30.96  & 32.69 & 33.04 & 32.87  & 32.66 \\\hline
\end{tabular}
\caption{Zh-En 4-ref dev BLEU w/ test-time wait-1 model}
\label{tab:w1}
\end{table}

\begin{table*}[!]\centering
\begin{tabular}{|l|c|c|c|c|c|c|}\hline
Task  & Model            & Wait-1 & Wait-3 & Wait-5 & Wait-7 & Wait-9 \\\hline
zh-en & Wait-k           &   2    &   3    &   4    &   4    & 4 \\\hline
zh-en & Test-time Wait-k &   5    &   5    &   5    &   4    & 5 \\\hline
en-zh & Wait-k           &   2    &   1    &   4    &   5    & 4 \\\hline
en-zh & Test-time Wait-k &   3    &   5    &   5    &   5    & 5 \\\hline
de-en & Wait-k           &   1    &   2    &   3    &   4    & 5 \\\hline
de-en & Test-time Wait-k &   4    &   4    &   5    &   4    & 5 \\\hline
en-de & Wait-k           &   3    &   3    &   3    &   4    & 5 \\\hline
en-de & Test-time Wait-k &   3    &   4    &   5    &   5    & 5 \\\hline
\end{tabular}
\caption{Redecoding window size}
\label{tab:window}
\end{table*}

\begin{table*}[!]\centering
\begin{tabular}{|l|c|c|c|c|c|c|}\hline
Task  & Model            & Wait-1 & Wait-3 & Wait-5 & Wait-7 & Wait-9 \\\hline
zh-en & Wait-k           &   10    &   15    &   7    &   5    & 5 \\\hline
zh-en & Test-time Wait-k &   3    &   3    &   3    &   3    & 3 \\\hline
en-zh & Wait-k           &   15    &   3    &   5    &   5    & 3 \\\hline
en-zh & Test-time Wait-k &   15    &   7    &   7    &   5    & 7 \\\hline
de-en & Wait-k           &   15    &   15    &   5    &   7    & 3 \\\hline
de-en & Test-time Wait-k &   15    &   5   &   3    &   5    & 3 \\\hline
en-de & Wait-k           &   7    &   7    &   3    &   5    & 3 \\\hline
en-de & Test-time Wait-k &   15    &   3    &   3    &   3    & 3 \\\hline
\end{tabular}
\caption{Beam size}
\label{tab:beam}
\end{table*}


\begin{figure*}
\begin{tabular}{cc}
\centering
  \includegraphics[width=7.cm]{figs/zh2en_test.pdf} & \centering
  \includegraphics[width=7.cm]{figs/en2zh_test.pdf}
\end{tabular}\\
\captionof{figure}{
  Translation quality against latency metrics on Chinese-to-English simultaneous translation.
}
\label{fig:zh2en}

\begin{tabular}{cc}
\centering
  \includegraphics[width=7.cm]{figs/de2en_test.pdf} & \centering
  \includegraphics[width=7.cm]{figs/en2de_test.pdf}
\end{tabular}\\[-0.3cm]
\captionof{figure}{
  Translation quality against latency metrics on English-to-German simultaneous translation.
}
\label{fig:de2en}
\end{figure*}
<<<<<<< HEAD

\begin{figure*}
\begin{tabular}{cc}
\centering
  \includegraphics[width=7.cm]{figs/zh2en_ap.pdf} & \centering
  \includegraphics[width=7.cm]{figs/en2zh_ap.pdf}
\end{tabular}\\
\captionof{figure}{
  Translation quality against latency metrics on Chinese-to-English simultaneous translation.
}
\label{fig:zh2en}

\begin{tabular}{cc}
\centering
  \includegraphics[width=7.cm]{figs/de2en_ap.pdf} & \centering
  \includegraphics[width=7.cm]{figs/en2de_ap.pdf}
\end{tabular}\\[-0.3cm]
\captionof{figure}{
  Translation quality against latency metrics on English-to-German simultaneous translation.
}
\label{fig:de2en}
\end{figure*}

\begin{figure*}
\begin{tabular}{cc}
\centering
  \includegraphics[width=7.cm]{figs/zh2en_rl.png} & \centering
  \includegraphics[width=7.cm]{figs/en2zh_rl.png}
\end{tabular}\\
\captionof{figure}{
  Translation quality against latency metrics on Chinese-to-English simultaneous translation.
}
\label{fig:zh2en}
\end{figure*}
=======
>>>>>>> 180b54d49eadebdec6a068ddfc8982e757ed8181

